Prompt Refinement with Image Pivot for Text-to-Image Generation

For text-to-image generation, automatically refining user-provided natural language prompts into the keyword-enriched prompts favored by systems is essential for the user experience. Such a prompt refinement process is analogous to translating the prompt from "user languages" into "system languages". However, the scarcity of such parallel corpora makes it difficult to train a prompt refinement model. Inspired by zero-shot machine translation techniques, we introduce Prompt Refinement with Image Pivot (PRIP). PRIP innovatively uses the latent representation of a user-preferred image as an intermediary "pivot" between the user and system languages. It decomposes the refinement process into two data-rich tasks: inferring representations of user-preferred images from user languages and subsequently translating image representations into system languages. Thus, it can leverage abundant data for training. Extensive experiments show that PRIP substantially outperforms a wide range of baselines and effectively transfers to unseen systems in a zero-shot manner.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/prompt_cases.tex <==
\newlength{\myimagewidth}
\setlength{\myimagewidth}{0.17\linewidth} % 设置您希望的全局宽度

\begin{table}[t]
\centering
\scriptsize
\caption{Prompt refinement examples.}
\label{tab:prompt_case_study}
\setlength{\tabcolsep}{3pt}
\scalebox{0.9}[0.9]{
\begin{tabular}{m{0.65\linewidth}cc}
\toprule
\textbf{Input Prompt} & \textbf{SD1.4~\cite{rombach2022high}} & \textbf{SDXL~\cite{podell2023sdxl}}  \\ 
\midrule
A monkey is pictured acting as a DJ. & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/monkey_dj/sd14.png}} & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/monkey_dj/sdxl.png}}  \\
\addlinespace[2pt] 
A monkey is pictured acting as a DJ., he is wearing headphones and has a large smile on his face, he is holding a record, he is at a rave, he is on the cover of a tourism pamphlet for the state of Florida, he is a resident DJ at a local nightclub
& 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/monkey_dj/sd14_prip.png}} & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/monkey_dj/sdxl_prip.png}} \\
\midrule
A Walter White funko pop figurine. & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/walter_white/sd14.png}} & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/walter_white/sdxl.png}}  \\
\addlinespace[2pt] 
A Walter White funko pop figurine., intricate, highly detailed, photorealistic, 4k, HDR, smooth, sharp focus, high resolution, award-winning photo, taken at the 2022 EPCOT International Flower and Food Festival & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/walter_white/sd14_prip.png}} & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/walter_white/sdxl_prip.png}} \\
\midrule
A mushroom house in a dark forest, with warm light emitting from its windows. & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/mushroom_house/sd14.png}} & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/mushroom_house/sdxl.png}}  \\
\addlinespace[2pt] 
A mushroom house in a dark forest, with warm light emitting from its windows., by Thomas Kinkade, colorful, vibrant, intricate, highly detailed, deviantart, artstation, by Lisa Frank, by Artgerm & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/mushroom_house/sd14_prip.png}} & 
\raisebox{-.5\height}{\includegraphics[width=\myimagewidth]{./prompt_case_study/mushroom_house/sdxl_prip.png}} \\
\bottomrule
\end{tabular}}
\end{table}


\let\myimagewidth\undefined


==> tables/refl_cases.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Images generated by different methods.}
\label{tab:image_case_study}
\setlength{\tabcolsep}{1pt}
\scalebox{0.9}[0.9]{
\begin{tabular}{cccc|cc}
\toprule
\textbf{SD1.4}~\cite{rombach2022high} & \textbf{+ReFL}~\cite{xu2023imagereward} & \textbf{+PRIP} & \textbf{+ReFL+PRIP} & \textbf{SDXL}~\cite{podell2023sdxl} & \textbf{+PRIP}  \\ 
\midrule
\multicolumn{6}{c}{A digital art depicting a chicken wearing a suit.}
\\
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/chicken_in_suit/sd14.png}} & 
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/chicken_in_suit/refl.png}} & 
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/chicken_in_suit/sd14_prip.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/chicken_in_suit/refl_prip.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/chicken_in_suit/sdxl.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/chicken_in_suit/sdxl_prip.png}} 
\\
\midrule 
\multicolumn{6}{c}{The interior of a spaceship orbiting alpha centauri.}
\\
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/spaceship_interior/sd14.png}} & 
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/spaceship_interior/refl.png}} & 
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/spaceship_interior/sd14_prip.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/spaceship_interior/refl_prip.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/spaceship_interior/sdxl.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/spaceship_interior/sdxl_prip.png}} 
\\
\midrule
\multicolumn{6}{c}{A horse and astronaut in one image.}
\\
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/astronount_horse/sd14.png}} & 
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/astronount_horse/refl.png}} & 
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/astronount_horse/sd14_prip.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/astronount_horse/refl_prip.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/astronount_horse/sdxl.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/astronount_horse/sdxl_prip.png}} 
\\
\midrule
\multicolumn{6}{c}{A plane flies in the sky passing over the moon.}
\\
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/plane_moon/sd14.png}} & 
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/plane_moon/refl.png}} & 
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/plane_moon/sd14_prip.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/plane_moon/refl_prip.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/plane_moon/sdxl.png}} &
\raisebox{-.5\height}{\includegraphics[width=0.17\linewidth]{./prompt_case_study/plane_moon/sdxl_prip.png}} 
\\
\bottomrule
\end{tabular}}
\end{table}

